Integrated modelling of microvibrations induced by Solar Array Drive Mechanism for worst-case end-to-end analysis and robust disturbance estimation

Modern and future observation Space missions face increasingly more demanding pointing performance requirements. This is accompanied with the development of larger lightweight flexible structures. This paper outlines a methodology for modeling a generic multi-body flexible spacecraft in an end-to-end fashion within the Two-Inputs Two-Outputs Port framework: from disturbance all the way to pointing performance by tacking into account all the uncertainties of each sub-system. A particular focus is dedicated to a novel generic model for Solar Drive Array Mechanisms and its harmonic disturbances produced by the micro-stepping driver and the gearbox imperfections. The proposed model is validated with the on-board telemetries of a European spacecraft. Moreover this paper shows how the proposed model-based approach can be easily used for control design and closed-loop robust performance analysis. Worst-case scenarios of mechanical parameters combination are investigated to provide robust performance certificate of the reference study case. A Linear Parameter-Varying observer, scheduled by the solar array rotor angle, is finally proposed in order to estimate the disturbance torques induced by the gearbox imperfections just using the measurements coming from a classical attitude control system: a star tracker and a gyrometer.

==> header.tex <==
\usepackage{verbatim}
\usepackage{xparse}

\usepackage{graphicx}

\usepackage[hyperref,dvipsnames]{xcolor}
\usepackage{color, colortbl}
\usepackage{transparent}
\usepackage{tcolorbox}
% for bold calligraphic math 
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{bm}

\usepackage{mathtools}
\usepackage{mleftright} % fix spacing after \left and \right
\DeclarePairedDelimiter\parentheses{\lparen}{\rparen}

% for colored bars in the captions
\usepackage{stackengine}
%\newcommand\crule[1][black]{\textcolor{#1}{\rule{10pt}{7pt}}}		
\DeclareDocumentCommand \crule
{  m o }{
\stackengine{0.5pt}{\textcolor{black}{\rule{\IfValueTF{#2}{#2}{10pt}}{6pt}}}{\textcolor{#1}{\rule{\IfValueTF{#2}{#2-1pt}{9pt}}{5pt}}}{O}{c}{F}{F}{L}	
}

% \usepackage{unicode-math}
\usepackage{enumitem}
\usepackage{import}
\usepackage{amsmath}
\usepackage{siunitx}

\usepackage[c]{esvect}

\usepackage{interval} % math intervals

\usepackage{booktabs}
\usepackage{multirow}

\usepackage{cuted}
\usepackage{framed}
\usepackage[super]{nth}

\definecolor{colorJSVlinks}{RGB}{51,126,177}
\usepackage[colorlinks]{hyperref}
\AtBeginDocument{
    \hypersetup{
        linkcolor=colorJSVlinks,
        citecolor=colorJSVlinks
    }
}
\usepackage[nameinlink]{cleveref}
\crefformat{equation}{(#2#1#3)}

% Captions
\usepackage{subcaption}
\renewcommand{\figurename}{Fig.}
\captionsetup[figure]{labelfont={bf},labelsep=period}
\captionsetup[subfigure]{labelfont=normalfont}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% centered plus-minus sign
\newcommand{\rpm}{\raisebox{.2ex}{$\scriptstyle\pm$}}

\DeclareDocumentCommand \bmf
{ m }{
	\bm{#1}
}

\DeclareDocumentCommand \coordframe
{  m m m m }{
\left(#1\,;#2,#3,#4\right)
}

\DeclareDocumentCommand \transportmat
{  m m o }{
\mf{\IfNoValueTF{#3}{T}{#3 T}}[#1#2]
}

\DeclareDocumentCommand \statespace{m m m m o}{%
\ensuremath{{\def\arraystretch{1.3}\IfValueTF{#5}{#5}{}\left(\begin{array}{c|c}
    #1 & #2 \\ \hline
    #3 & #4
\end{array}\right)}}
}

% Refine suppremum operator
\let\sup\relax
\DeclareMathOperator*{\sup}{\text{sup}}
\DeclareMathOperator*{\mininimize}{\text{minimize}}
\let\log\relax
\DeclareMathOperator*{\log}{\text{log}}
\let\det\relax
\DeclareMathOperator*{\det}{\text{det}}
\let\min\relax
\DeclareMathOperator*{\min}{\text{min}}

% Title of a paragraph
\DeclareDocumentCommand \partitle
{ m }{
\textbf{\textit{#1:}}\quad
}

%% RHinf set
\DeclareDocumentCommand \rhinf
{  o o } {%
\mathbb{RH}_\infty\IfValueTF{#1}{^{#1 \times #2}}{}%
}

\newcommand{\ts}{%
\intercal%\mathsf{T}
}
\newcommand{\simnew}{\approx\!}
\DeclareDocumentCommand \SmallBmatrix
{ m o } {
		\ensuremath{
		\begingroup
		%\normalsize
		%\small
		\IfNoValueTF{\footnotesize}{#2}
		\arraycolsep=0.1\arraycolsep
		\renewcommand*{\arraystretch}{0.3}
		\begin{bmatrix}#1\end{bmatrix}
		\endgroup
	}
}

\newcommand\SmallMatrix[1]{{%
		\ensuremath{
			\begingroup
			%\normalsize
			\small
			\arraycolsep=0.1\arraycolsep
			\renewcommand*{\arraystretch}{0.3}
			\begin{matrix}#1\end{matrix}
			\endgroup
}}}

% L2 
% \DeclareDocumentCommand \ltwo{ o } {
% %\mathcal{L}_2\IfValueTF{#1}{^{#1}}{}
% \mathbb{L}\IfValueTF{#1}{^{\!#1}}{}
% }

\DeclareDocumentCommand \hinf{ m } {\left\|#1\right\|_\infty}

%% INLINE VECTOR
\DeclareDocumentCommand \iv
{  m o  } {%
{\IfNoValueTF{#2}{\footnotesize}{#2}
\arraycolsep=2pt\def\arraystretch{1}
\left[
\begin{matrix}
#1
\end{matrix}
\right]}%
}


\DeclareDocumentCommand \smax
{  m o o } {%
	\IfNoValueTF{#2}{%
	\overline{\sigma}\left(#1\right)%
	}{%
	\overline{\sigma}#2#1#3
	}
}
\DeclareDocumentCommand \smin
{  m o o } {%
	\IfNoValueTF{#2}{%
	\underline{\sigma}\left(#1\right)%
	}{%
	\underline{\sigma}#2#1#3
	}
}

% \newcommand{\tf}[2]{{#1 \rightarrow #2}}
\newcommand{\tf}[2]{{#1 \rightarrow #2}}

\DeclareDocumentCommand \vf
{  m O{} o } {%symbf instead of boldsymbol for xelatex
	\mathbf{#1}_{#2}\IfNoValueTF{#3}{}{\{#3\}}%
}
\DeclareDocumentCommand \vfs
{  m O{} o } {%symbf instead of boldsymbol for xelatex
	\mathbf{#1}_{#2}\IfNoValueTF{#3}{}{\{#3\}}%
    %\mathbf{#1}_{#2}
}
\DeclareDocumentCommand \mf
{  m O{} O{} } {%symbf instead of boldsymbol for xelatex
	%\mathbf{#1}_{#2}
% 	\symbf{#1}_{#2}
    \mathbf{#1}_{#2}
}

\DeclareDocumentCommand \Ts
{  m } {%
%\mathbb{T}\left({#1}\right)
%\mathbb{T}({#1})
\mathbf{\mathcal T}({#1})
}

\DeclareDocumentCommand \eye
{  O{} } {%
	\mathbf{I}_{#1}%
}
\DeclareDocumentCommand \zeros
{ o o } {
	\mathbf{0}_{		
		\IfNoValueTF{#1}{}{#1}
		\IfNoValueTF{#2}{}{\times#2}		
	}
}
% \DeclareDocumentCommand \fu
% { o o }{\mathcal{F}_u
% \IfNoValueTF{#1}{}{\left({#1},{#2}\right)}}
% \DeclareDocumentCommand \fu
% { o o }{\IfNoValueTF{#1}{{\color{red}HERE}}{\left({#2} \star {#1}\right)}}
\DeclareDocumentCommand \starprod
{ m m o o}{\IfNoValueTF{#3}{\left(}{#3}{#1} \star {#2}\IfNoValueTF{#4}{\right)}{#4}}
\DeclareDocumentCommand \fu
{ o o }{{\color{red}\textbf{HERE}}}

\DeclareDocumentCommand \fl
{ o o }{
	\mathcal{F}_l%
    \IfNoValueTF{#1}{}{%
    	\IfNoValueTF{#2}{}{%
%        	\,\left({#1},{#2}\right)
            \left({#1},{#2}\right)%
% 			\left(\begingroup #1 \endgroup,\begingroup #2 \endgroup\right)%
        }%
    }% 
}

\DeclareDocumentCommand \muDD
{ o }{
	\mu_
	{\IfNoValueTF{#1}{\mf{\Delta}}{#1}}
}
\DeclareDocumentCommand \muD
{ o o }{
	\muDD[#2]	
    \IfNoValueTF{#1}{}{
	\left(#1\right)}
}


\newcommand{\diag}{\text{diag}\!}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc}
\DeclareDocumentCommand \circled
{ m o }{
    \tikz[baseline=(char.base)]{
        \node[shape=circle,fill=white,draw,inner sep=\IfNoValueTF{#2}{2pt}{#2}] (char) {#1};
    }
}


\definecolor{colorA1}{RGB}{10,22,221}
\definecolor{colorA2}{RGB}{153,0,0}
\definecolor{colorL}{RGB}{26,0,128}
\newcommand*\nodecircle[1]{\tikz{\fill[#1] (0,0)circle (1.5pt);
\draw[#1] (0,0)circle (2.3pt);
}}
\newcommand*\nodesquare[1]{\tikz{\fill[#1] (-1.4pt,-1.4pt)rectangle ++(2.8pt,2.8pt);
\draw[#1] (0,0)circle (2.3pt);
}}
\newcommand*\nodetriangle[1]{\tikz{\fill[#1] (0pt,2.0pt)--(-1.7321pt,-1.0pt)--(1.7321pt,-1.0pt);
\draw[#1] (0,0)circle (2.3pt);
}}

                    
% Real and imaginary parts of a complex number
\newcommand{\ReV}{\mathrm{Re}}
\newcommand{\ImV}{\mathrm{Im}}            
            
% Line numbers            
%\usepackage[switch,pagewise]{lineno}

% Redefine widehat
\newcommand{\newtilde}[1]{\hat{#1}}
\newcommand{\newhat}[1]{\check{#1}}
\newcommand{\newbar}[1]{\tilde{#1}}


% underbar
\newcommand{\ubar}[1]{\mkern 1.5mu\underline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\uubar}[1]{\ubar{\ubar{#1}}}
% overbar
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

% differential operator
\DeclareDocumentCommand \diff
{ o } {
		\mathop{}\!\mathrm{
			\IfNoValueTF{#1}{d}{d{#1}}
	}
	%\IfNoValueTF{#1}{\mathop{d}}{\mathop{d#1}}
}

% imaginary number sqrt(-1)
\newcommand{\jimag}{\textrm{j}}
